RelatIF: Identifying Explanatory Training Examples via Relative Influence

In this work, we focus on the use of influence functions to identify relevant training examples that one might hope "explain" the predictions of a machine learning model. One shortcoming of influence functions is that the training examples deemed most "influential" are often outliers or mislabelled, making them poor choices for explanation. In order to address this shortcoming, we separate the role of global versus local influence. We introduce RelatIF, a new class of criteria for choosing relevant training examples by way of an optimization objective that places a constraint on global influence. RelatIF considers the local influence that an explanatory example has on a prediction relative to its global effects on the model. In empirical evaluations, we find that the examples returned by RelatIF are more intuitive when compared to those found using influence functions.

==> computational.tex <==
%----------------------------------------------------------------------
\section{Efficiently Computing Influence}
%----------------------------------------------------------------------
\TBD{
\begin{itemize}
    \item Although there are many interesting applications for IFs, their computational complexity are a significant barrier.
    \item This is especially true if we want to use IFs to produce explanations at inference time. 
    \item One approximate inverse HVP and a search through the training gradients requires at least 3 epochs worth of computation. (In practice we find much more is required.)
    \item Where $NP$ parameters fit in memory we can store $[H+ \lambda I]^{-1} G$, and inference time explanations become possible; but otherwise we need another approach.
    \item An alternative approach has been to treat all but the last layer as constant. (Somewhat justifiable, but it deviates considerably from true IF).
    \item Ultimately we ne $q: \Reals^P \mapsto \Reals^N$ which executes quickly, fits in memory and where $q(\nabla l_{\text{test}}) \approx G^T [H+ \lambda I]^{-1} \nabla l_{\text{test}}$
    \item In searching for $q$ we can draw on two areas of existing research: second order optimization, 
    \item last layer or block-diagonal approximation for hessian
    \begin{itemize}
        \item showing the changes in the accuracy of the estimation as we freeze more layers (moving from input to the classifier)
        \item reduction of the number of model parameters: freezing vs. layer-wise hessian computation
    \end{itemize}
\end{itemize}
}

While influence functions offer promising insights into how machine learning models are affected by their training data, their computational intensity is a significant barrier in their use. 
Even with the inverse Hessian vector product (HVP) approximations suggested by Koh such as LiSSA, and CG, computing influence in larger machine learning models is very slow.
The inverse HVP methods suggested requires a minimum of an epoch worth of mini-batch HVP applications to approximate $s_{\text{test}} = H^{-1}\nabla l_{\text{test}}$.
This is followed by an another epoch of worth of gradient computations to search for the most influential training points: those maximizing (or minimizing) $ s_{\text{test}} \cdot \nabla l_{\text{train}}$.
Assuming we can compute mini-batch HVPs in roughly 2-3 times what it takes to compute mini-batch gradients ( possible with access to both forward and reverse mode AD), finding the most influential training points for a given test point requires at least 3 epochs worth of gradient computations. 
This is much to slow to provide an explanation at inference.

Computing influence functions at inference time would be possible if we had a function $q: \Reals^P \mapsto \Reals^N$ which fit in memory and which, given the gradient of the test point of interest, promptly returned the influence of every point in the training set.
In small models where fitting $NP$ parameters in memory is possible, $q(\nabla l_{\text{test}})$ can be set to exactly $G^T H^{-1} \nabla l_{\text{test}}$, where G is a $P$ by $N$ matrix where the i\textsuperscript{th} column is $\nabla l_i$, the gradient of the i\textsuperscript{th} training point.
However, in large models storing $NP$ parameters could easily require upwards of 10 or even 100 of terabytes of memory. 
We can nonetheless hope to find 

We propose a novel approach to computing influence that further reduces the memory and compute requirements. 




At the root of this approach is a dimensionality reduction. Using principal component analysis (PCA) we identify the directions that explain the majority of the variance among the pointwise training loss gradients, and project them into a lower dimensional space spanned by these high-variance directions. 
This projection allows us to make accurate influence function approximations with less than 10\% of the original model dimensions.
We also propose a slight modification to the LiSSA algorithm which reduces variance and eliminates the needs to average over several approximations. 

In order to evaluate the quality of our approximations, we consider three performance metrics. 1) The correlation between the influence as computed by our method and that computed using the full Hessian. 2) The normalized discounted cumulative gain (NDCG): a measure of the approximation's ability to recall the most influential points, and 3) the mean squared error (MSE) of the self influence scores. 

\subsection{IF in fewer dimensions}
Let $\theta = A\omega$, where $\theta$, the model parameters, are $ \in \Reals^P$, $\omega \in \Reals^Q$, and $Q << P$. We then have $\nabla_\omega L = A^T \nabla_\theta L$, and $\nabla^2_\omega L = A^T [\nabla^2_\theta L] A$. If we let A be the top Q eigenvectors of $\sum_{i=1}^N \nabla_\theta L_i \nabla_\theta L_i^T$ (i.e. co-variance of the point-wise loss gradients, a.k.a the empirical Fisher), we have that $\nabla_\omega L$ is the most accurate Q-dimensional representation of $\nabla_\theta L$ (in the sense that it minimizes the $l_2$ reconstruction error). 

We can compute $A$ after training the model using incremental PCA, and $\nabla^2_\omega L$ can be computed exactly with only $Q$ Hessian vector products (HVP), which do not require forming $\nabla^2_\theta L$ explicitly. 

\begin{itemize}
    \item Modern neural network models often operate in an over-parameterized regime. 
    \item Previous IF work has considered only a subset of model parameters with successful results (brunet, koh)
    \item 
\end{itemize}



\section{Optimal Projection}

Let $\theta \in \Reals^D$ be the parameters, and $A \in \Reals^{d \times D}$ some projection matrix. Let $H$ denote the Hessian of the empirical risk, and $g_i \in  \Reals^D$ be the gradient of the loss evaluated at the $i^{\mathrm{th}}$ data point $z_i$, i.e. $g_i = \grad_{\theta} \loss (z_i, \theta )$.

The influence function between two data points $z_i$ and $z_j$ is denoted as $\Infl{i}{j}$. Similarly, we define $\InflP{i}{j}{A}$ as
\[
\InflP{i}{j}{A}=   g_i^T (A^{\dagger} A)^{T} H^{-1} A^{\dagger} A g_j ,
\]

\TBD{GKD: Project in the parameter space and compute the Hessian via chain rule.}

which is the influence function between data points $z_i,z_j$ in a projected subspace.,
Letting $H^{-1}_A =  (A^{\dagger} A)^{T} H^{-1} A^{\dagger} A $, the expression can be rewritten as
\[
\InflP{i}{j}{A} = g_i^T H^{-1}_A g_j.
\]

Our goal is to find a projection matrix $A^*$ minimizing an average squared error between $\Infl{i}{j}$ and $\InflP{i}{j}{A}$, i.e., 
\[
A^*  = \arg \min_{A \in \Reals^{d \times D} \,:\, \mathrm{rank}(A)=d } \frac{1}{m^2} \sum_{i,j} (\Infl{i}{j} - \InflP{i}{j}{A})^2.
\]
Expanding the square and getting rid of the terms not depending on $A$ gives us
\[
A^*=\arg \min_{A} \sum_{i,j}  \Infl{i}{j}^{A,2} - 2  \InflP{i}{j}{A} \Infl{i}{j} .
\]
Since $ \InflP{i}{j}{A}$ is a scalar and due to the cyclic property of the trace, 
\begin{align}
\Infl{i}{j}^{A,2} &= \trace \Big( \InflP{i}{j}{A}  \InflP{i}{j}{A}  \Big)\\
&= \trace \Big(  g_i^T H^{-1}_A g_j g_j^T H^{-1 \, T}_A g_i \Big) \\
&= \trace \Big(  g_i g_i^T H^{-1}_A g_j g_j^T H^{-1\, T}_A \Big) \\
&= \trace \Big(  G_i H^{-1}_A G_j H^{-1 \, T}_A  \Big),
\end{align}

\TBD{
EB: eq (6) to (8): why do we have ``transposed'' $H^{-1}_A$ at the end?
}

where $G_i = g_i g_i^T $.

Similarly, since $ \Infl{i}{j} $ is also a scalar, we obtain:
\begin{align}
    2  \InflP{i}{j}{A} \Infl{i}{j} &=  2 \trace \Big(  G_i H^{-1}_A G_j H^{-1\, T}  \Big) \\
    &= 2 \trace \Big(  G_i H^{-1}_A G_j H^{-1\, T}_A  \Big),
\end{align}
\TBD{Explain the last equality}.

Let $G = \frac{1}{m} \sum_{i} G_i$. Then
\begin{align}
A^* &=  \arg \min_{A} \trace \Big( \sum_{i,j} \Infl{i}{j}{A,2} - 2  \InflP{i}{j}{A} \Infl{i}{j} \Big) \\ 
&= \arg \min_{A} \trace \Big( - G H^{-1}_A G H^{-1\, T}_A \Big) \\
&= \arg \max_{A} \trace \Big( G H^{-1}_A G H^{-1\, T}_A \Big).
\end{align}

\TBD{GKD: Discuss diagonal case.}

\TBD{GKD: Discuss the case were cov matrix is equal to the hessian.}

\TBD{GKD: Can we implement an approximation of this?}

\TBD{M-E: $H^{-1}_A$ is symmetric I think...}


==> headers.tex <==
% !TEX root =  main.tex

%\usepackage{amsaddr}
\usepackage[utf8]{inputenc} 
\usepackage{amsthm,amsmath, amssymb,bm, amsfonts, cases, mathtools, thmtools}
\usepackage{verbatim}
\usepackage{graphicx}\graphicspath{{figures/}}
\usepackage{multicol}
\usepackage{tabularx}
%\usepackage[usenames,dvipsnames]{xcolor}
% \usepackage{mathrsfs} 
%\usepackage{url}
% %\usepackage{caption}
\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
%\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage[%
    minnames=1,maxnames=99,maxcitenames=3,
    style=authoryear,%alphabetic, %numeric,
    sortcites=true,
    doi=false,url=false,
    giveninits=true,
    hyperref,natbib,backend=biber]{biblatex}
    
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
\bibliography{biblio}
%\usepackage[numbers]{natbib}
%\bibliographystyle{acmtrans-ims}

\defbibenvironment{bibliography}
  {\trivlist}
  {\endtrivlist}
  {\item
   \printtext[labelnumberwidth]{%
     \printfield{labelprefix}%
      \printfield{labelnumber}}%
   \addspace}


\usepackage{datetime}

%% change up the fonts for fun.
%\usepackage[OT1]{eulervm} 
%\usepackage{palatino}

\DeclareMathAlphabet\EuRoman{U}{eur}{m}{n}
\SetMathAlphabet\EuRoman{bold}{U}{eur}{b}{n}
\newcommand{\eurom}{\EuRoman}

%% hide equation numbers for unreferenced equations
%\mathtoolsset{showonlyrefs}

%% make text prettier
%\usepackage{euscript,microtype}
%\DisableLigatures{encoding = *, family = * }

\usepackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=RawSienna]{hyperref}
%\usepackage{hypernat}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}


%% nicer way of making \ref'ences to theorems, lemmas, equations, sections, etc.
\usepackage[capitalize]{cleveref}

%% add entries for anything missing.
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{theorem}{Theorem}{Theorems}

%% grey out the equation numbers slightly
\makeatletter
\let\reftagform@=\tagform@
\def\tagform@#1{\maketag@@@{\ignorespaces\textcolor{gray}{(#1)}\unskip\@@italiccorr}}
\renewcommand{\eqref}[1]{\textup{\reftagform@{\ref{#1}}}}
\makeatother

%% theorem styles
\declaretheorem[style=plain,numberwithin=section,name=Theorem]{theorem}
\declaretheorem[style=plain,sibling=theorem,name=Lemma]{lemma}
\declaretheorem[style=plain,sibling=theorem,name=Proposition]{proposition}
\declaretheorem[style=plain,sibling=theorem,name=Corollary]{corollary}

\declaretheorem[style=definition,sibling=theorem,name=Definition]{definition}
%\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem,name=Example]{example}
%\declaretheorem[style=remark,qed=$\triangleleft$,sibling=theorem,name=Remark]{remark}
%\declaretheorem[style=definition,qed=$\triangleleft$,sibling=theorem]{fact}

%\numberwithin{equation}{section}
\numberwithin{theorem}{section}

\renewcommand{\appendixname}{}
%\renewcommand{\sectionname}{\S}

%% put ruler down the side for draft, and color it gray
%\input{myvruler.tex}

